Best of Both Worlds: Transferring Knowledge from Discriminative Learning to a Generative Visual Dialog Model

We present a novel training framework for neural sequence models, particularly for grounded dialog generation. The standard training paradigm for these models is maximum likelihood estimation (MLE), or minimizing the cross-entropy of the human responses. Across a variety of domains, a recurring problem with MLE trained generative neural dialog models (G) is that they tend to produce 'safe' and generic responses ("I don't know", "I can't tell"). In contrast, discriminative dialog models (D) that are trained to rank a list of candidate human responses outperform their generative counterparts; in terms of automatic metrics, diversity, and informativeness of the responses. However, D is not useful in practice since it cannot be deployed to have real conversations with users. Our work aims to achieve the best of both worlds -- the practical usefulness of G and the strong performance of D -- via knowledge transfer from D to G. Our primary contribution is an end-to-end trainable generative visual dialog model, where G receives gradients from D as a perceptual (not adversarial) loss of the sequence sampled from G. We leverage the recently proposed Gumbel-Softmax (GS) approximation to the discrete distribution -- specifically, an RNN augmented with a sequence of GS samplers, coupled with the straight-through gradient estimator to enable end-to-end differentiability. We also introduce a stronger encoder for visual dialog, and employ a self-attention mechanism for answer encoding along with a metric learning loss to aid D in better capturing semantic similarities in answer responses. Overall, our proposed model outperforms state-of-the-art on the VisDial dataset by a significant margin (2.67% on recall@10). The source code can be downloaded from https://github.com/jiasenlu/visDial.pytorch.

==> more_figure.tex <==
\begin{table}[t]
    \vspace{-6pt}
	\renewcommand*{\arraystretch}{0.8}
    \setlength{\tabcolsep}{6px}
    \caption{Qualitative comparison.}
    \label{table:qualititve} 
    \begin{center}\hspace{-5.5pt}
    \begin{tabular}{p{3.0cm} p{2.6cm} p{2cm} p{2.1cm} p{2.1cm}}
    \toprule
    \scriptsize Image+Caption & {\scriptsize Question} & \scriptsize GT Answer & \scriptsize G-MLE Answer & \scriptsize G-DIS Answer \\
    \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3} \cmidrule(l){4-4}\cmidrule(l){5-5}
    % First
    \vspace{-32pt}
    \center
    \includegraphics[width=2.2cm]{figure/507065.jpg}
    \newline\vspace{-15pt}
    \begin{minipage}{3.2cm}
    \begin{compactenum}[\hspace{-6pt}]
    \tiny
    \item \tiny A little boy sitting on a wooden bench eating half a sandwich.
    \end{compactenum}
    \end{minipage}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item Is the photo in color? 
    \item About how old is the boy?
    \item Can you tell what kind of sandwich he is eating?
    \item Is the shirt plain green or is there a design or character on it?
    \item Is he eating by himself? 
    \item Is the outside or inside? 
    \item Is he sitting at a table? 
    \item Is it sunny outside? 
    \item Can you see anyone else in the photo?
    \item 
    \end{compactenum}}
    \end{minipage}}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item Male 
    \item Male 
    \item Black
    \item UNK and pant with shoes
    \item Luggage bag
    \item Yes
    \item Yes, it is snow mountain
    \item Yes
    \item No
    \item Not sure
    \end{compactenum}}
    \end{minipage}}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item I can't tell
    \item I can't tell
    \item Brown
    \item Black jacket
    \item A small 1
    \item Yes
    \item Yes
    \item Yes
    \item No
    \item yes    
    \end{compactenum}}
    \end{minipage}}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item Male
    \item Can't tell
    \item Brown
    \item Snowsuit
    \item Backpack
    \item Yes
    \item Yes
    \item Yes
    \item Yes
    \item Can't tell 
    \end{compactenum}}
    \end{minipage}}
    \\
    \midrule	    
    \vspace{-32pt}
    \center
    \includegraphics[width=2.2cm]{figure/52462.jpg}
    \newline\vspace{-13pt}
    \begin{minipage}{3.2cm}
    \begin{compactenum}[\hspace{-6pt}]
    \tiny
    \item \tiny Two zebra standing next to each other in a dry grass field.
    \end{compactenum}
    \end{minipage}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item Are zebras in zoo? 
    \item Are they adults or babies?
    \item Are they standing next to each other? 
    \item Is there water source in image? 
    \item Is it sunny out? 
    \item Any trees? 
    \item Are zebras eating?  
    \item Any other animals in picture? 
    \item Is there any type of enclosure?
    \item Is grass green?
    \end{compactenum}}
    \end{minipage}}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item No zebras not in zoo 
    \item I would say they are adults 
    \item 1 lead in front , while other 1
    \item No
    \item It does look like sunny 
    \item There are few trees but is not in 
    \item No , they are walking 
    \item No
    \item No
    \item No
    \end{compactenum}}
    \end{minipage}}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item No
    \item They are adult
    \item Yes they are
    \item No water 
    \item Yes
    \item Yes, many trees
    \item No, they are just standing around
    \item No
    \item No
    \item Yes    
    \end{compactenum}}
    \end{minipage}}
    &
    \resizebox{4cm}{!}{
    \begin{minipage}{3in}{
    \begin{compactenum}[\hspace{-4pt}]
    \item No
    \item They appear to be adult 
    \item Yes they are 
    \item I do not see any water 
    \item Yes it is  
    \item Yes, lots of trees in background 
    \item No they are not eating 
    \item No just zebras 
    \item No
    \item Yes
    \end{compactenum}}
    \end{minipage}} 
    \\
    \bottomrule
    \end{tabular}\\%[5pt]
    \end{center}
    \vspace{-4mm}
\end{table}
